PruneTrain: Fast Neural Network Training by Dynamic Sparse Model Reconfiguration

State-of-the-art convolutional neural networks (CNNs) used in vision applications have large models with numerous weights. Training these models is very compute- and memory-resource intensive. Much research has been done on pruning or compressing these models to reduce the cost of inference, but little work has addressed the costs of training. We focus precisely on accelerating training. We propose PruneTrain, a cost-efficient mechanism that gradually reduces the training cost during training. PruneTrain uses a structured group-lasso regularization approach that drives the training optimization toward both high accuracy and small weight values. Small weights can then be periodically removed by reconfiguring the network model to a smaller one. By using a structured-pruning approach and additional reconfiguration techniques we introduce, the pruned model can still be efficiently processed on a GPU accelerator. Overall, PruneTrain achieves a reduction of 39% in the end-to-end training time of ResNet50 for ImageNet by reducing computation cost by 40% in FLOPs, memory accesses by 37% for memory bandwidth bound layers, and the inter-accelerator communication by 55%.

==> Makefile <==
all:  main.tex bib/*.bib acmart.cls
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex -synctex=-1 main
	sed -i -e 's/build_tex/tex/g' -e 's/\/cygdrive\/c/C:/g' main.synctex
	#gs -sOutputFile=main_bw.pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -dNOPAUSE -dBATCH main.pdf
clean: 
	rm -rf *.aux *.bbl *.blg *.log *.out main.pdf main_bw.pdf main.dvi main.synctex


==> tex/eval_imagenet.tex <==
\subsection{\squeezetrain on a Large Dataset}
\label{sec:eval_imagenet}

We train and prune ResNet50 and VGG16 on ImageNet from scratch using \squeezetrain with different regularization penalty ratios. We use the same number of training iterations (90 epochs) for both baseline dense training and \squeezetrain without any retraining (detaching regularization) after pruning.

As compared to the dense baseline training, PruneTrain reduces the total training FLOPs by 29\% and the end-to-end training time by 17\% using TITAN Xp GPU and 18\% using TESLA V100 GPU.
Also, compared to the dense baseline, it reduce the inference FLOPs by 41\% losing a minor accuracy as shown in \tab{tab:imagenet_table}.

\begin{table}[h]
    \caption{ResNet50 training results on ImageNet with PruneTrain.}
    \vspace*{1.0mm}
    \centering
    \noindent\resizebox{0.95\linewidth}{!}{
        \tabulinesep=0.95mm
        \renewcommand{\arraystretch}{0.7}
        \begin{tabu}{cccc}
            \thickhline
            \makecell{Baseline\\Val. Acc.} & \makecell{Val. \\Acc. \(\Delta\)} & \makecell{Inference \\FLOPs} & \makecell{Train. FLOPs \\(E2E time TITAN Xp/V100)}  \tabularnewline
            \midhline
            76.2\%                         & -1.5\%                            & 59\%                         & 71\% (83 / 82\%)   \tabularnewline
            \thickhline
        \end{tabu} 
    }
    \label{tab:imagenet_table}
    \vspace*{-3mm}
\end{table}


\noindent\textbf{Computation and Memory Cost Reduction During Training.}
% Learning the structure by regularization => Retrained with XX epochs but no accuracy imporovement. This means we learned the structured and weights by a one shot training

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{graph/imagenet_train_cost.pdf}
    \vspace*{-5mm}
    \caption{XXXXX.}
    \label{fig:imagenet_train_cost}
\end{figure}

\noindent\textbf{Communication Cost Saving at Distributed Training.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.42\textwidth]{graph/imagenet_comm_cost.pdf}
    \vspace*{-3mm}
    \caption{XXXXX.}
    \label{fig:imagenet_comm_cost}
\end{figure}

\noindent\textbf{Parameter Compression.}

\noindent\textbf{Retraining Without Regularization To Recover Accuracy.}
%Lose parameter compression rate for accuracy
